Representation Online Matters: Practical End-to-End Diversification in Search and Recommender Systems

As the use of online platforms continues to grow across all demographics, users often express a desire to feel represented in the content. To improve representation in search results and recommendations, we introduce end-to-end diversification, ensuring that diverse content flows throughout the various stages of these systems, from retrieval to ranking. We develop, experiment, and deploy scalable diversification mechanisms in multiple production surfaces on the Pinterest platform, including Search, Related Products, and New User Homefeed, to improve the representation of different skin tones in beauty and fashion content. Diversification in production systems includes three components: identifying requests that will trigger diversification, ensuring diverse content is retrieved from the large content corpus during the retrieval stage, and finally, balancing the diversity-utility trade-off in a self-adjusting manner in the ranking stage. Our approaches, which evolved from using Strong-OR logical operator to bucketized retrieval at the retrieval stage and from greedy re-rankers to multi-objective optimization using determinantal point processes for the ranking stage, balances diversity and utility while enabling fast iterations and scalable expansion to diversification over multiple dimensions. Our experiments indicate that these approaches significantly improve diversity metrics, with a neutral to a positive impact on utility metrics and improved user satisfaction, both qualitatively and quantitatively, in production. An accessible PDF of this article is available at https://drive.google.com/file/d/1p5PkqC-sdtX19Y_IAjZCtiSxSEX1IP3q/view

==> Skintone_Diversification_2/macros.tex <==
\newcommand{\as}[1]{\textcolor{blue}{[Ashudeep: #1]}}
\newcommand{\ps}[1]{\textcolor{blue}{[Pedro: #1]}}
\newcommand{\nf}[1]{\textcolor{blue}{[Nadia: #1]}}
\newcommand{\sd}[1]{\textcolor{blue}{[Shloka: #1]}}
\newcommand{\bj}[1]{\textcolor{blue}{[Bhawna: #1]}}
\newcommand{\reviewedit}[1]{\textcolor{blue}{#1}}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\newcommand{\DiversitySet}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\metric}[2]{\ensuremath{\text{Div}@{#1}(#2)}\xspace}
\newcommand{\RankingSystem}{\ensuremath{R}\xspace}
\newcommand{\QuerySet}{\ensuremath{\mathcal{Q}\xspace}}
\newcommand{\kmax}{K_{\max}}

%DPP Params
\newcommand{\DPPBatchSize}{\ensuremath{B}\xspace}
\newcommand{\DPPDepth}{\ensuremath{N'}\xspace}
\newcommand{\DPPWindowSize}{\ensuremath{w}\xspace}


% Methods
\newcommand{\StrongOR}{\textsc{Strong-OR}\xspace}
\newcommand{\OverfetchAndRerank}{\textsc{Overfetch-and-Rerank}\xspace}
\newcommand{\SmartOverfetch}{\textsc{Smart-Overfetch}\xspace}
\newcommand{\DPPLong}{\textsc{Determinantal Point Process}\xspace}
\newcommand{\DPP}{\textsc{DPP}\xspace}
\newcommand{\RRLong}{\textsc{Round-Robin}\xspace}
\newcommand{\RR}{\textsc{RR}\xspace}
\newcommand{\BucketizedANN}{\textsc{Bucketized-ANN} Retrieval\xspace}
\newcommand{\MMRLong}{\textsc{Maximal Marginal Relevance}\xspace}
\newcommand{\MMR}{\textsc{MMR}\xspace}

% Surfaces
\newcommand{\PDP}{Related Products\xspace}
\newcommand{\Search}{Search\xspace}
\newcommand{\Homefeed}{Homefeed\xspace}
\newcommand{\NUX}{New User Homefeed\xspace}


